Medical Bill Shock and Imperfect Moral Hazard

Consumers are sensitive to medical prices when consuming care, but delays in price information may distort moral hazard. We study how medical bills affect household spillover spending following utilization, leveraging variation in insurer claim processing times. Households increase spending by 22\% after a scheduled service, but then reduce spending by 11\% after the bill arrives. Observed bill effects are consistent with resolving price uncertainty; bill effects are strongest when pricing information is particularly salient. A model of demand for healthcare with delayed pricing information suggests households misperceive pricing signals prior to bills, and that correcting these perceptions reduce average (median) spending by 16\% (7\%) annually.

==> Sections/model-results.tex <==
We estimate the model presented in Section \ref{sec:model} for 240,111 households in our analytical sample enrolled in plans with nonzero deductibles from 2006 to 2013. For each household-week, we simulate household health shocks and draw household moral hazard parameters; then, for different values of $\beta$, we estimate household signals of underlying OOP spending and associated marginal costs, $\hat{c}_{it}$. Taken together, these estimates produce a prediction of spending $m_{it}(\beta)$, which differs as $\beta$ changes. Our primary measure of model fit is the root mean squared error (RMSE) between observed and predicted levels of weekly spending at the household level. 

\input{figtex/fig_model1results}

Figure \ref{fig:model1-results} presents the estimated relationship between $\beta$ and model fit, based on 50 simulations with different individual health shocks. The median RMSE for each value of $\beta$, as well as a confidence band of two standard deviations, are shown. Increasing the guess of $\beta$ reduces the RMSE until the function reaches a minimum at $\beta=1.104$ (in the median simulation), after which RMSE increases. The blue band in the figure shows the estimated 95\% confidence region for the minimizing value of $\beta$, $[1.101,1.107]$. This implies households over-estimate the OOP spending of services prior to the arrival of price information by between 10.1\% and 10.7\%, consistent with the findings of Section \ref{sec:rf-evidence}. 

We conduct a counterfactual analysis to compare how spending predictions differ given this inflation, against a counterfactual world where $\beta$ is correctly perceived to be 1 for all household-weeks (see Appendix Figure \ref{fig:cost-cf-m1} for details on the simulation). We find that over-estimating the costs of medical services leads to over-spending for 11.9\% of households, with the average (median) affected household spending \$856 (\$486) more per household member in medical services that they would not have selected had they been correctly informed of their true OOP costs. This corresponds to an over-spending of 34.8\% (33.1\%) for the average (median) affected household (see Section \ref{subsec:cfs} below for more details).\footnote{Note that these percentage changes are measured relative to the counterfactual predicted spending; that is, as $(Actual - Counterfactual)/Counterfactual$.} 

\subsection{Learning} 

We also incorporate household learning about $\beta$ over time into our model. The median household's prior for $\beta$ is roughly 1.75, indicating an 75\% over-estimate of OOP costs (95\% bootstrapped CI: [1.702,1.798]). There is relatively little variation across households; the estimated prior variance parameter is $\sigma^2_{\beta,0}=0.011$ (95\% CI: [0.002, 0.020]). Put into context, we estimate that 95.5\% of households (two standard deviations on either side of the mean) have priors in the interval $(1.54, 1.96)$, indicating high levels of under-information.\footnote{Note that given the estimated mean and standard deviation of prior beliefs, fewer than 5e-11\% of households would be expected to have beliefs of $\beta \leq 1$.}

\input{figtex/fig_learning}

Figure \ref{fig:learning} shows how beliefs evolve in response to medical spending. We estimate that bills provide extremely precise information, with the signal variance term estimated to be 0.0002 (95\% CI: [-8e-5,.0005]). That is, roughly 95.5\% of household signals for $\beta$ fall in the interval $(0.97, 1.03)$. This leads to rapid convergence of beliefs as the year progresses, as illustrated in the figure in the blue curve, which indicates the average value of $\hat{\beta}$ across the sample by week of year. However, convergence stalls after the first quarter---it isn't until week 33 that the average household's value of $\beta$ crosses 1.107 (the upper bound of the static confidence interval), and average beliefs don't dip below 110\% until week 45.\footnote{The average household does not have sufficiently many medical encounters for their beliefs to converge completely; by the end of the plan-year, the average household value of $\beta$ is estimated to be about 1.094, just outside of the confidence interval for the $\beta$ in the non-learning model. Appendix Figure \ref{figax:misinformation} presents further results illustrating heterogeneity in beliefs across a year.}

% \subsection{Counterfactual Exercises}\label{subsec:cfs}

% The full model with household learning permits the same counterfactual simulations as above. We estimate predicted spending differences between the observed data (using the equilibrium model parameters) and three counterfactual states of the world: one where consumers are fully informed about their OOP costs at the time of service ($\beta=1$ for all household-weeks); one where priors are re-centered around the truth ($\mu_{\beta,0}=1$, but the other learning parameters remain unchanged); and one where deductibles reset more frequently than at the yearly level. While the first counterfactual exercise assumes full information, in the second exercise beliefs are centered around $\beta=1$ but drawn randomly, with decreasing uncertainty over time. Finally, the exercises in which deductibles reset more frequently capture changes in both how often household uncertainty affects the estimated marginal costs of services and the length of time for which uncertainty is allowed to persist. 

% \input{Tables/Counterfactuals}

% Table \ref{tab:cfs} presents the results.\footnote{See also Appendix Figure \ref{fig:cost-cf-m1} for a distribution of estimated spending differences.} The information in the first two rows of the table repeats the counterfactual exercise reported in discussion of the non-learning model above. Compared to the first two rows of Panel B, we find that allowing for household learning results in a greater fraction of individuals who over-spend while waiting for bills to arrive. This makes intuitive sense, given that households restricted to no learning in the simpler model may have been estimated to have reasonably correct beliefs for the full plan year, when in fact they experienced a period of rapid learning (and over-spending) early in the year. Compared to a state where $\beta$ is fixed at 1, roughly 21\% of households over-consume care, with the average (median) affected household consuming \$1,051 (\$575) more per household member. This corresponds to an over-spending of 44.4\% (40.8\%) for the average (median) household relative to the predicted spending under full information. 

% This over-spending is almost entirely attributed to high household priors, as shown in row 3 of Panel B of the table. Re-centering household priors---without completely eliminating residual uncertainty around prices for each unique medical event---accounts for more than 95\% of the over-spending for both the average and median household. 

% \subsubsection{Optimal Deductible Design with Under-information}\label{subsubsec:ded-reset}
% In addition to simulating spending with real-time information or learning, we also conduct simulations that assess the role of plan design in mitigating over-consumption arising from price delays. Given that over-consumption is most prevalent when households incorrectly believe that they have met a deductible, we first evaluate the tradeoffs associated with policies that shorten a deductible's effective period. This is a potential solution which has recently been proposed by health policy experts \citep{shafer_monthly_2022}.

% Shortening the length of a deductible trades off a reduced intensity of uncertainty---through both shorter periods of uncertainty and overall lower levels of a deductible---against the possibility of more frequent periods of uncertainty.\footnote{The intuition for this tradeoff is illustrated in Appendix Figure \ref{fig:dedreset-intuition}.} That is, with a lower deductible that resets more frequently, patients may be induced to over-spend even following low-cost medical procedures.\footnote{When shortening the length of the deductible period by a factor $c < 1$, actuarially fair deductibles decrease by a factor $c' \in (c, 1)$; that is, deductibles do not decrease at a one-to-one replacement rate. We calculate new deductibles at actuarially fair rates while holding premiums constant \citep{hong_time_2022}. In our case, the quarterly deductible is 30.75\% of the annual, while the monthly deductible is 10.25\%.} In addition, a lower threshold for changes in marginal costs may induce greater levels of \textit{ex-post} moral hazard, particularly in short periods of time where medical care can be highly concentrated, such as after a shoppable health service. 

% We model these trade-offs in policy simulations considering how consumption may change when deductibles are applied annually, quarterly, and monthly. Table \ref{tab:cfs} reports results for both the learning and non-learning models. We find that as deductibles reset more frequently, consumers are expected to nearly double their chosen levels of consumption: the average (median) household increases their consumption by 81\% (92\%) per-person in the non-learning model (Panel A) and 77\% (89\%) in the learning model (Panel B). Note that this arises principally due to moral hazard concerns concentrated in the relatively short lengths of time following a large health expense shock (either expected or scheduled); hence, we do not observe large differences in predicted spending increases as deductibles move from quarterly to monthly, or after incorporating learning into our model. 

% \subsubsection{Heterogeneity in Responses}

% Table \ref{tab:cfs} appears to suggest that, particularly after allowing household belief updating, shortened deductible periods only affect spending on the extensive margin and do little to mitigate the spending effects of delayed information. However, these results mask significant time heterogeneity across households, given that some learn more rapidly about $\beta$ than others. We report how our simulations affect these families differently by stratifying households by the quartile of their total number of visits in a year. % The results presented in Table \ref{tab:cfs} conflate households with limited spending in a year (and hence, limited information about prices) and households who incur more frequent bills. Households are grouped in quartiles: those with the fewest visits are shown below in red (2 or fewer visits), while those in the highest quartile are shown in blue (9 or more visits). The middle two quartiles of the distribution include households with between 3 and 8 visits annually.

% % While shortening deductible periods increases overall spending, the policy appears to have limited effectiveness in reducing the over-consumption from delayed information. In the absence of learning, the incidence of over-consumption drops to 8.5\% (nearly a 30\% decrease from 11.9\%), with the average (median) household's over-consumption dropping by 24\% (26\%). However, when beliefs evolve, there is no reduction in over-spending; instead, over-spending appears to increase on the extensive margin (as suggested in Figure \ref{fig:dedreset-intuition}). This over-consumption is more limited in scope: when deductibles reset monthly, the average (median) over-spending drops to \$714 (\$404) per person, down 32\% (20\%) from baseline. 

% \input{figtex/fig_quarters.tex}

% Figure \ref{fig:quarters} presents the results when deductibles reset quarterly.\footnote{Over-spending is the spending difference between the model and a counterfactual where $\beta=1$.} Panel (a) shows the incidence of over-consumption from delayed claim adjudication---that is, how under-informed beliefs about $\beta$ drive spending. In the first quarter, households have similar beliefs about $\beta$, meaning only those with higher spending tend to over-consume. We observe the top 75\% of the distribution is almost twice as likely to over-consume care than the bottom quartile. However, as the year progresses, high-spending families also refine their beliefs about costs, which reduces overspending to as little as 2\% in the fourth quarter. Low-spending households who do not learn about $\beta$ continue to over-spend at high rates throughout the year. Similar results are apparent along the intensive margin in panel (b).\footnote{In the first quarter, poor beliefs about $\beta$ drive over-consumption for high-spending households; the top quartile has predicted over-spending 33\% higher than those in the bottom quartile. This difference vanishes over time as beliefs refine; by the end of the plan year, the median amount of overspending is similar across all affected households, roughly \$300.}

% Our simulations therefore suggest households better informed about $\beta$ benefit more from shortened deductible periods, driven mainly by reductions in the extensive margin of over-consumption. By the last quarter of the year---when $\beta \approx 1.1$---information uncertainty only causes overspending for 4\% of households. Taken together, the results of our model and counterfactual simulations corroborate the reduced-form findings in Section \ref{sec:rf-evidence}: households over-estimate their actual OOP expenditures while awaiting bills, leading to overspending for many households. Overspending is more pronounced when households have less information about prices, and may be mitigated by more frequent signals, shorter waiting periods for bills, or shorter deductible periods. 

==> Tables/BillBalanceTable_20220915.tex <==
% latex table generated in R 4.2.1 by xtable 1.8-4 package
% Thu Sep 15 11:24:56 2022
\begin{table}[ht]
\centering
\begin{threeparttable}
\begin{tabular}{|l|cc|cc|c|cc|}
  \hline  & \multicolumn{2}{c|}{\textbf{Average Spending}} & \multicolumn{2}{c|}{\textbf{Difference}} & & \multicolumn{2}{c|}{\textbf{Sample Size}} \\
Procedure & $d\leq30$ & $d>$30 & Unadjusted & Adjusted & $p$-value & $d\leq30$ & $d>$30 \\ 
  \hline
Removal, prostate & \$21,834 & \$25,362 & \$3,528 & \$1,260 & 0.41 & 917 & 403 \\ 
Removal, knee cartilage & \$7,619 & \$8,021 & \$402 & \$697 & 0.00 & 46,937 & 15,606 \\ 
Removal, breast growth & \$4,887 & \$5,173 & \$286 & \$674 & 0.00 & 10,550 & 3,916 \\ 
Injection, anesthetic & \$3,258 & \$3,537 & \$279 & \$484 & 0.00 & 49,604 & 16,667 \\ 
Biopsy, esophagus/stomach & \$3,317 & \$3,238 & -\$79 & \$406 & 0.00 & 245,411 & 65,603 \\ 
Removal, tonsils (age $<$ 12) & \$4,578 & \$4,871 & \$293 & \$342 & 0.00 & 21,503 & 4,962 \\ 
Shaving, shoulder bone & \$12,262 & \$12,040 & -\$222 & \$233 & 0.07 & 27,952 & 11,410 \\ 
Biopsy, prostate & \$2,653 & \$2,377 & -\$276 & \$124 & 0.01 & 23,172 & 6397 \\ 
Removal, gallbladder & \$9,217 & \$9,794 & \$577 & \$96 & 0.38 & 36,756 & 13,252 \\ 
Hernia repair & \$6,753 & \$6,724 & -\$28 & \$28 & 0.83 & 14,314 & 5,215 \\ 
Removal, cataract (no insertion) & \$1,408 & \$1,198 & -\$210 & -\$179 & 0.05 & 11,776 & 2,388 \\ 
Vaginal delivery & \$7,789 & \$7,927 & \$139 & -\$344 & 0.00 & 82,968 & 36,068 \\ 
Removal, cataract (lens insertion) & \$6,114 & \$5,958 & -\$156 & -\$346 & 0.00 & 43,129 & 9,266 \\ 
Vaginal delivery, prior C-section & \$8,429 & \$8,634 & \$205 & -\$912 & 0.01 & 1298 & 503 \\ 
   \hline
\end{tabular}
\begin{tablenotes}
    \small
    \item \textit{Notes:} Table shows differences in means for total spending (patient + insurer payments) by procedure category for the shoppable services included in our analytical sample. Services are divided into groups if (1) the bill took 30 days or fewer to arrive following the service ($d \leq 30$) or (2) the bill took more than 30 days to arrive ($d > 30$). Differences in means are presented both in raw, unadjusted terms, as well as adjusted for provider-specific fixed-effects. $p$-values are the results of two-way difference in means testing on the adjusted differences. 
\end{tablenotes}
\caption{\label{tab:balance} Bill Balance Table (Unadjusted and Adjusted for Provider Fixed Effects)} 
\end{threeparttable}
\end{table}


==> Tables/DistributionRegTable_pay_asinh.tex <==
\begin{table}[htbp] \centering
\newcolumntype{C}{>{\centering\arraybackslash}X}

\label{tab:distreg}
\begin{tabularx}{0.85\linewidth}{l|cccc}

\toprule
Distribution &\multicolumn{2}{c}{Event Cost} & \multicolumn{2}{c}{Pre-Event Annual Spending} \tabularnewline
Unit& Total Cost& OOP & Total&OOP  \tabularnewline
\midrule
Service&3.99**&4.03**&4.34**&4.13** \tabularnewline
&(0.01)&(0.01)&(0.01)&(0.01) \tabularnewline
Service x Quantile\_1&--0.04**&--0.15**&0.21**&0.36** \tabularnewline
&(0.01)&(0.01)&(0.01)&(0.01) \tabularnewline
Service x Quantile\_2&0.03*&--0.05**&0.16**&0.32** \tabularnewline
&(0.01)&(0.01)&(0.01)&(0.01) \tabularnewline
Service x Quantile\_3&0.03*&--0.12**&0.09**&0.15** \tabularnewline
&(0.01)&(0.01)&(0.01)&(0.01) \tabularnewline
Service x Quantile\_4&0.03**&--0.04**&--0.01&--0.03** \tabularnewline
&(0.01)&(0.01)&(0.01)&(0.01) \tabularnewline
Service x Quantile\_6&--0.04**&0.05**&--0.29**&--0.19** \tabularnewline
&(0.01)&(0.01)&(0.01)&(0.01) \tabularnewline
Service x Quantile\_7&--0.01&0.06**&--0.47**&--0.27** \tabularnewline
&(0.01)&(0.01)&(0.01)&(0.01) \tabularnewline
Service x Quantile\_8&--0.03*&0.07**&--0.64**&--0.36** \tabularnewline
&(0.01)&(0.01)&(0.01)&(0.01) \tabularnewline
Service x Quantile\_9&--0.04**&0.07**&--0.80**&--0.55** \tabularnewline
&(0.01)&(0.01)&(0.01)&(0.01) \tabularnewline
Service x Quantile\_10&0.07**&0.19**&--1.10**&--0.88** \tabularnewline
&(0.01)&(0.01)&(0.01)&(0.01) \tabularnewline
\midrule
Bill&0.30**&0.22**&0.38**&0.58** \tabularnewline
&(0.01)&(0.01)&(0.01)&(0.01) \tabularnewline
Bill x Quantile\_1&0.05**&0.08**&0.15**&--0.04** \tabularnewline
&(0.01)&(0.01)&(0.01)&(0.01) \tabularnewline
Bill x Quantile\_2&0.00&0.27**&0.05**&--0.11** \tabularnewline
&(0.01)&(0.01)&(0.01)&(0.01) \tabularnewline
Bill x Quantile\_3&--0.02&0.07**&--0.02&--0.10** \tabularnewline
&(0.01)&(0.01)&(0.01)&(0.01) \tabularnewline
Bill x Quantile\_4&--0.01&--0.01&--0.06**&--0.07** \tabularnewline
&(0.01)&(0.01)&(0.01)&(0.01) \tabularnewline
Bill x Quantile\_6&0.04**&0.03*&--0.11**&--0.12** \tabularnewline
&(0.01)&(0.01)&(0.01)&(0.01) \tabularnewline
Bill x Quantile\_7&0.02&0.07**&--0.11**&--0.21** \tabularnewline
&(0.01)&(0.01)&(0.01)&(0.01) \tabularnewline
Bill x Quantile\_8&0.06**&0.09**&--0.12**&--0.31** \tabularnewline
&(0.01)&(0.01)&(0.01)&(0.01) \tabularnewline
Bill x Quantile\_9&0.09**&0.13**&--0.16**&--0.37** \tabularnewline
&(0.01)&(0.01)&(0.01)&(0.01) \tabularnewline
Bill x Quantile\_10&0.04**&0.11**&--0.24**&--0.43** \tabularnewline
&(0.01)&(0.01)&(0.01)&(0.01) \tabularnewline
\midrule
$R^2$&0.44&0.44&0.46&0.46 \tabularnewline
$N$&42,271,702&42,271,702&42,271,702&42,271,702 \tabularnewline
\bottomrule 

\end{tabularx}
\end{table}


==> Tables/OLDCounterfactuals.tex <==
\begin{table}[htb]
\centering
\begin{threeparttable}
\begin{tabular}{lcc|ccc}
\toprule
& \multicolumn{2}{c}{Spending/Person} & &  \multicolumn{2}{c}{Conditional Differences}\\\cmidrule{2-3}\cmidrule{5-6}
& \multicolumn{1}{c}{Average} & \multicolumn{1}{c}{Median} & \multicolumn{1}{c}{\% Diff $> 0$} &  \multicolumn{1}{c}{Average} & \multicolumn{1}{c}{Median}  \\
\midrule
\multicolumn{2}{l}{\textbf{Panel A: Non-Learning Model}} \\ 
Observed Data & \$2,001 & \$1,123 & -- & -- & --  \\
Full Information ($\beta$ = 1) & \$1,899 & \$1,066 & 11.9\% & \$856 & \$486 \\
Deductible Resets Quarterly & \$3,499 & \$2,040 & 12.7\% & \$751 & \$424 \\
Deductible Resets Monthly & \$3,745 & \$2,272 & 8.5\% & \$657 & \$361 \\ 
\midrule
\multicolumn{2}{l}{\textbf{Panel B: Learning Model}} \\ 
Observed Data & \$2,119 & \$1,181 & -- & -- & --  \\
Full Information ($\beta$ = 1) & \$1,899 & \$1,068 & 21.0\% & \$1,051 & \$575 \\
Re-centered Priors ($\mu_{\beta,0}=1$) & \$1,896 & \$1,065 & 21.7\% & \$1,031  &\$562 \\
Deductible Resets Quarterly & \$3,662 & \$2,135 & 29.9\% & \$863 & \$477 \\
Deductible Resets Monthly & \$3,851 & \$2,335 & 22.7\% & \$714 & \$404 \\ 
\bottomrule
\end{tabular}
\begin{tablenotes}
    \small
    \item \textit{Notes}: Table presents average and median spending per household member predicted under different assumptions placed on structural parameters. Panel A uses the base model (Section \ref{subsec:model-simple}) and Panel B incorporates learning (Section \ref{subsec:model-learning}). The first row in each panel indicates predicted spending using empirical data; subsequent rows impose assumptions on parameters in counterfactual scenarios. These include full information without learning (row 2), learning with re-centered priors (row 3, panel B only), and policies shortening the length of a deductible. Shortened deductibles are calculated at actuarially fair rates while holding premiums constant (quarterly deductibles are 30.75\% of annual deductibles; monthly deductibles are 10.25\%)---see \cite{hong_time_2022} for a discussion. All currencies are reported in 2022 USD. 
    \end{tablenotes}
    \caption{\label{tab:cfs} Comparison of Predicted Spending Across Counterfactual States of the World}
\end{threeparttable}
\end{table}


==> Tables/OLDServiceRegs_DDDtable.tex <==
\begin{table}[p]
\centering
\begin{threeparttable}
\begin{tabular}{l|cc|cc}
\toprule
& \multicolumn{2}{c}{\textbf{Regression Coefficients}} & \multicolumn{2}{c}{\textbf{Pre-Treatment Averages}} \\
& \multicolumn{1}{c}{Post Service} & \multicolumn{1}{c}{Post Bill} &\multicolumn{1}{c}{\% $\geq 0 $} & \multicolumn{1}{c}{Conditional Mean} \\
\midrule
\textbf{Hospital Care} \\
Emergency Department &  0.108*** & -0.021 & 0.67\% &      \$929.98 \\
& (0.0129) & (0.0133) \\
Preventable Hospitalizations &  0.371*** & -0.194* & 0.04\% &  \$19,979.89 \\
& (0.0829) & (0.0848) \\
\midrule
\textbf{Outpatient Care} \\
Behavioral Health & -0.02 &  0.018 & 1.19\% &     \$119.47  \\
& (0.0132) & (0.0134) \\
Chiropractic Care & -0.005 &  0.027 & 1.86\% &    \$133.39 \\
& (0.0147) & (0.0151) \\
% Durable Medical Equipemnt &  0.353*** & -0.260*** & 0.37\% &     \$236.54 \\
% & (0.0278) & (0.0284) \\
Evaluation \& Management &  1.440*** & -0.518*** &1.05\%  &     \$121.45\\
& (0.0066) & (0.0062) \\
Imaging &  0.098*** & -0.037*** & 2.55\%  &     \$265.52 \\
& (0.0108) & (0.0111) \\
Lab Services &  0.198*** & -0.178*** & 3.96\% &      \$62.14  \\
& (0.0113) & (0.0119) \\
Low-Value Services &  0.084*** &  0.028** & 6.58\% &     \$148.61 \\
& (0.0094) & (0.0097) \\
Preventive Care &  0.345*** & -0.249*** & 11.68\% &     \$120.47  \\
& (0.0036) & (0.0037) \\
Specialist Care &  0.550*** & -0.181*** & 0.57\% &     \$114.70 \\
& (0.0192) & (0.0198) \\
\midrule
\textbf{Prescriptions} &  0.018*** & -0.006 & 18.30\% &     \$147.14  \\
& (0.0047) & (0.0048) \\
\bottomrule
\end{tabular}
\begin{tablenotes}
\small
\item \textit{Notes}: Table shows coefficients from triple-difference regressions capturing service-specific effects of pricing information ($N=59,177,995$). Columns (1) and (2) present regression coefficients; column (3) indicates the fraction of pre-treatment weeks when spending was positive; and column (4) presents pre-treatment weekly averages, conditional on positive spending. See Appendix Table A.2 for a complete list of the CPT codes for each of the outpatient categories. $^{*} p < 0.05, ^{**} p < 0.01, ^{***} p < 0.001$
\end{tablenotes}
\caption{\label{tab:services} Estimated Impact of Bill Arrival on Service-Specific Spending}
\end{threeparttable}
\end{table}


==> Tables/SummaryTable_Household_Slides.tex <==
\begin{table}[htbp]
\centering
\begin{threeparttable}
\begin{tabular}{l|cc}
\toprule
& \multicolumn{1}{c}{Full Sample} & \multicolumn{1}{c}{Plan-Identified Sample} \\
\midrule
Total spending & \$4,764 [\$975] (0.002) & \$4,406 [\$887] (0.002) \\
\% with 0 spending & 0.17 (0.000) & 0.20 (0.000) \\
OOP spending & \$650 [\$198] (0.000) & \$562 [\$167] (0.000) \\
Deductible $|$ $>0$ & --- & \$1,040.24 (0.001) \\
\% with 0 deductible & --- & 0.26 (0.000) \\
\% w/ shoppable services & 0.06 (0.000) & 0.06 (0.000) \\
\hspace{.25cm} Total cost & \$5,572 [\$3,721] (0.011) & \$5,645 [\$3,814] (0.015) \\
\hspace{.25cm} OOP & \$691 [\$388] (0.002) & \$574 [\$290] (0.002) \\
\midrule
Years & 2006--2018 & 2006--2013 \\
$N_\text{families}$ & 368,237 &367,445 \\
$N_\text{individuals}$ & 1,357,392 & 1,311,554 \\
\bottomrule
\end{tabular}
\end{threeparttable}
\end{table}


==> figtex/axfig_ESBillArrival.tex <==
\begin{figure}[p]
    \caption{Dynamic Effects of Bill Arrival on Spillover Household Medical Spending}
    \label{axfig:es-bill}
    \centering
    
    \includegraphics[width=7.0in]{Figures/AppendixFigure_EventStudy_BillArrival_20230710.pdf}
    \vspace{0.2cm}

    \begin{minipage}{0.95\textwidth} 
	{\footnotesize \textit{Notes}: Figure shows regression coefficients from TWFE Poisson regressions estimating the dynamic treatment effects of a bill's arrival relative to pre-bill, post-service spending. Regressions are limited to weeks after the shoppable service is consumed and use not-yet-treated households as the control group; regressions include fixed effects for year and week-of-year of shoppable service as well as service types and physicians. Coefficients are recentered relative to the week prior to a bill's arrival, to account for the fact that spending coefficients are mechanically higher post-service. The DDD coefficient estimated in Table \ref{tab:ddd-table} is presented as a horizontal dashed line for reference.
	\par
	}
	\end{minipage}
\end{figure}


==> figtex/axfig_rawdata.tex <==
\begin{figure}[p]
    \caption{Variation in Spillover Spending by Week of Bill Arrival}
    \label{axfig:rawdata}
    \centering
    
    \subfloat[Raw Data]{
	    \includegraphics[width=3.0in]{Figures/AppendixFigure_RTS_20230708.pdf}
	 }
	\subfloat[Shoppable Service Event Studies]{
	    \includegraphics[width=3.0in]{Figures/AppendixFigure_EventStudies_20230711.pdf}
	 }
    \vspace{0.2cm}

    \begin{minipage}{0.95\textwidth} 
	{\footnotesize \textit{Notes}: Figures show differences in estimated spillover spending (at the weekly level) in both the raw data and as regression coefficients from two-way fixed-effects (TWFE) regressions with the shoppable service consumption as the treatment. Spending for three groups is shown: those whose bill arrives in the same week as the same service and those whose bill is delayed by one or four weeks, respectively. Vertical dashed lines indicate bill arrivals. TWFE regressions account for household, year, week-of-year, and provdier fixed-effects, and cluster standard errors at the individual level.
	\par
	}
	\end{minipage}
\end{figure}


==> figtex/fig_counterfactualspending_m1.tex <==
\begin{figure}[p]
    \caption{Counterfactual Analysis: Change in Predicted Spending from Correcting $\beta = 1$}
    \label{fig:cost-cf-m1}
    \centering
    
    \subfloat[No Learning Model]{
	    \includegraphics[width=3.0in]{Figures/Model1_CounterfactualSpending.pdf}
	 }
	\subfloat[Learning Model]{
	    \includegraphics[width=3.0in]{Figures/Model2_CounterfactualSpending.pdf}
	 }
    \vspace{0.2cm}

    \begin{minipage}{0.95\textwidth} 
	{\footnotesize \textit{Notes}: Figure shows estimated the differences in predicted (total) per-person health spending that arise from requiring that $\beta = 1$ in Equation \ref{eq:beta}, rather than the parameters estimated in the models  (see Figure \ref{fig:model1-results}). Panel (a) shows results for the model without learning while panel (b) shows results for the generalized learning model. Histogram displays distribution of household-year average differences per person, conditional on a difference greater than 0. Note that for 87.5\% of households in panel (a) and 77.6\% of households in panel (b), no differences in spending are predicted. The dashed line indicates the average conditional difference in per-person spending while the dot-dashed line indicates the median in both groups.
	\par
	}
	\end{minipage}
\end{figure}


==> figtex/fig_dedreset.tex <==
\begin{figure}[htbp]
    \caption{Effect of Resetting Deductible More Frequently on Demand Uncertainty}
    \label{fig:dedreset-intuition}
    \centering

	    % Figure notes: https://towardsdatascience.com/using-pgfplots-to-make-economic-graphs-in-latex-bcdc8e27c0eb
        \begin{tikzpicture}
        \begin{groupplot}[
        group style={
            group size=1 by 2,
            horizontal sep=0pt,
            vertical sep = 1.5pt,
        },
        width=0.9\textwidth,
        height=0.45\textwidth,
        grid=both,
        xmin = -11, xmax = 11, ymin=-5,
        % ymin = -4, ymax = , 
        xtick = \empty, ytick = \empty, 
        axis lines*=none,
        hide axis, 
        clip = false
    ]
    \nextgroupplot[title=Panel A: No Deductible Resetting]
        % \begin{axis}[
        % xmin = -11, xmax = 11, ymin = -5, ymax = 5, 
        % xtick=\empty, ytick=\empty,
        % axis lines*=none,
        % hide axis,
        % clip = false % Allows me to label outside graph
        % ]
        % Labels
        % \node [right] at (current axis.above origin) {Deductible Reset};
        % \node [below] at (-10,-2) {$t_0$};
        % \node [below] at (10,-2) {$t_1$};
        
        % Boundary Lines 
        % \addplot[domain = -10:-2, restrict y to domain = -2:2, samples = 400, color = blue]{1};
        % \addplot[domain = -10:-2, restrict y to domain = -2:2, samples = 400, color = blue]{-1};
        % \addplot[domain = 2:10, restrict y to domain = -2:2, samples = 400, color = red]{1};
        % \addplot[domain = 2:10, restrict y to domain = -2:2, samples = 400, color = red]{-1};
        % \addplot[domain = -2:2, restrict y to domain = -2:2, samples = 400, color = purple]{1};
        % \addplot[domain = -2:2, restrict y to domain = -2:2, samples = 400, color = purple]{-1};
        \addplot[domain = -11:11, restrict y to domain = -2:2, samples = 400, color = black,thick]{0};

        % Vertical Lines 
        
        % Labels for functions
        \node [below] at (-6,-2) {\textcolor{blue}{Know $M < d_1$}};
        \node [below] at (6,-2) {\textcolor{red}{Know $M > d_1$}};
        \node [below] at (0, -3) {\textcolor{purple}{Uncertainty about $M$}};
        \draw[color=purple] (0,-3) to (0,-1.25);
        
        % Dashed lines
        \addplot[color = black, thick] coordinates {(-10,-1.5) (-10,1.5)}; % Far left boundary
        \addplot[color = black, thick] coordinates {(10,-1.5) (10,1.5)}; % Far right boundary
        \addplot[color = blue, thick] coordinates {(-2,-1.5) (-2,1.5)}; % Service date
        \addplot[color = red, thick] coordinates {(2,-1.5) (2,1.5)}; % Bill date
                \node [above] at (-2,1.5) {\textcolor{blue}{Service}};
        \node [above] at (2,1.5) {\textcolor{red}{Bill}};
        
        % Fill Regions and label
        \fill[red, opacity = 0.1] (2,1) -- (10,1) -- (10,-1) -- (2,-1);
        \fill[blue, opacity = 0.1] (-10,-1) -- (-10,1) -- (-2,1) -- (-2,-1);
        \fill[purple, opacity = 0.1] (-2,1) -- (2,1) -- (2,-1) -- (-2,-1); 
        % \node at (.75,9) {$P_2$};
        % \node at (4.15,9) {$P_1$};
        % \node at (8.25,9) {$P_0$};
        
        % \end{axis}

        \nextgroupplot[title=Panel B: Deductible Resetting]
        
        % \begin{axis}[
        % xmin = -11, xmax = 11, ymin = -5, ymax = 5, 
        % xtick=\empty, ytick=\empty,
        % axis lines*=none,
        % hide axis,
        % clip = false % Allows me to label outside graph
        % ]
        % Labels
        % \node [right] at (current axis.above origin) {Deductible Reset};
        % \node [below] at (-10,-2) {$t_0$};
        % \node [below] at (10,-2) {$t_1$};
        
        % Boundary Lines 
        % \addplot[domain = -10:-2, restrict y to domain = -2:2, samples = 400, color = blue]{1};
        % \addplot[domain = -10:-2, restrict y to domain = -2:2, samples = 400, color = blue]{-1};
        % \addplot[domain = 2:10, restrict y to domain = -2:2, samples = 400, color = red]{1};
        % \addplot[domain = 2:10, restrict y to domain = -2:2, samples = 400, color = red]{-1};
        % \addplot[domain = -2:0, restrict y to domain = -2:2, samples = 400, color = purple]{1};
        % \addplot[domain = -2:0, restrict y to domain = -2:2, samples = 400, color = purple]{-1};
        \addplot[domain = -11:11, restrict y to domain = -2:2, samples = 400, color = black,thick]{0};

        % Vertical Lines for deductible reset
        \addplot[color = black, dashed, very thick] coordinates {(0,-2.5) (0,2.5)}; % Deductible reset
        
        % Labels for functions
        \node [below] at (-6,-2) {\textcolor{blue}{Know $M < d_2$}};
        \node [below] at (3,-2) {\textcolor{blue}{Know $M < d_2$}};
        \node [below] at (8,-3) {\textcolor{purple}{Uncertainty about $M$}};
        \node [below] at (-1, -3) {\textcolor{purple}{Uncertainty about $M$}};
        \draw[color=purple] (-1,-3) to (-1,-1.25); 
        \draw[color=purple] (8,-3) to (8,-1.25); 
        
        % Dashed lines
        \addplot[color = black, thick] coordinates {(-10,-1.5) (-10,1.5)}; % Far left boundary
        \addplot[color = black, thick] coordinates {(10,-1.5) (10,1.5)}; % Far right boundary
        \addplot[color = blue, thick] coordinates {(-2,-1.5) (-2,1.5)}; % Service date
        \node [above] at (-2,1.5) {\textcolor{blue}{Service 1}};
        \addplot[color = blue, thick] coordinates {(6,-1.5) (6,1.5)}; % Service date
        \node [above] at (6,1.5) {\textcolor{blue}{Service 2}};
        \addplot[color = red, dashed, thin] coordinates {(2,-1.5) (2,1.5)}; % Bill date
        \node [above] at (2,1.5) {\textcolor{red}{Bill 1}};
        % \node [above] at (2,3) {\textbf{Deductible Resets}}; 
        % \draw[color=black,thick] (2,3) to (0,2.5);
        
        % Fill Regions and label
        \fill[purple, opacity = 0.1] (6,1) -- (10,1) -- (10,-1) -- (6,-1);
        \fill[blue, opacity = 0.1] (-10,-1) -- (-10,1) -- (-2,1) -- (-2,-1);
        \fill[purple, opacity = 0.1] (-2,1) -- (0,1) -- (0,-1) -- (-2,-1); 
        \fill[blue, opacity = 0.1] (6,1) -- (0,1) -- (0,-1) -- (6,-1); 
        % \node at (.75,9) {$P_2$};
        % \node at (4.15,9) {$P_1$};
        % \node at (8.25,9) {$P_0$};
        
        % \end{axis}
        \end{groupplot}
        \end{tikzpicture}
	 
    \vspace{0.2cm}
    \begin{minipage}{0.95\textwidth} 
	{\footnotesize \textit{Notes}: Figure illustrates the intuition behind the tradeoffs associated with deductibles of varying lengths. Larger deductibles covering a longer period of time may induce greater levels of uncertainty at specific, high-cost medical events (panel A); on the other hand, deductibles which reset more often (panel B) limit the over-consumption associated with a single period of uncertainty, but potentially induce multiple points across a plan year at which individuals are uncertain about whether or not they have met a deductible. Blue vertical lines indicate the point at which services are received which households may expect to change their marginal costs of future care (e.g., as deductibles are met), while red vertical lines indicate the bill arrival date. The dashed vertical line in panel B indicates the point at which the deductible resets within the plan-year.
	\par
	}
	\end{minipage}
\end{figure}


==> figtex/fig_quarters.tex <==
\begin{figure}[tbp]
    \caption{Heterogeneous Effects of Resetting Deductibles Quarterly on Over-Spending}
    \label{fig:quarters}
    \centering
    
    \subfloat[Extensive Margin]{
	    \includegraphics[width=3.0in]{Figures/Model2_QuarterOverSpending_ExtensiveMargin.pdf}
	 }
	\subfloat[Intensive Margin]{
	    \includegraphics[width=3.0in]{Figures/Model2_QuarterOverSpending_IntensiveMargin.pdf}
	 }
    \vspace{0.2cm}

    \begin{minipage}{0.95\textwidth} 
	{\footnotesize \textit{Notes}: Figure shows estimated differences in predicted per-person spending between two models where deductibles reset quarterly: the equilibrium parameters estimated in the learning model (Section \ref{subsec:model-learning}), and a counterfactual model where $\beta = 1$ across all individuals and periods. Quarterly deductibles are 30.75\% of the annual deductible, calculated at actuarially fair rates while holding premiums constant. Spending is stratified by the number of health encounters a household has had within a plan-year---those in the lowest quartile of number of medical visits are shown in red (group 1; 2 or fewer visits), while those in the highest quartile are in blue (group 3; 9 or more visits). Panel (a) shows results for the probability of any over-spending, while panel (b) shows the conditional median level of over-spending. 95\% confidence intervals are shown. 
	\par
	}
	\end{minipage}
\end{figure}

